BWS: Best Window Selection Based on Sample Scores for Data Pruning across Broad Ranges

Data subset selection aims to find a smaller yet informative subset of a large dataset that can approximate the full-dataset training, addressing challenges associated with training neural networks on large-scale datasets. However, existing methods tend to specialize in either high or low selection ratio regimes, lacking a universal approach that consistently achieves competitive performance across a broad range of selection ratios. We introduce a universal and efficient data subset selection method, Best Window Selection (BWS), by proposing a method to choose the best window subset from samples ordered based on their difficulty scores. This approach offers flexibility by allowing the choice of window intervals that span from easy to difficult samples. Furthermore, we provide an efficient mechanism for selecting the best window subset by evaluating its quality using kernel ridge regression. Our experimental results demonstrate the superior performance of BWS compared to other baselines across a broad range of selection ratios over datasets, including CIFAR-10/100 and ImageNet, and the scenarios involving training from random initialization or fine-tuning of pre-trained models.

==> figs/pruning_exp/pruning_exp.tex <==
\begin{figure*}[!tb]
\centering
    \includegraphics[width=0.98\linewidth]{figs/legend.pdf} \\
    \vspace{-0.6em}
    \subfigure[CIFAR-10 \label{fig:pruning_CIFAR10}]{\includegraphics[width=0.245\linewidth]{figs/pruning_exp/pruning_measure_CIFAR10_resnet18_no_iter.pdf}}
    \subfigure[CIFAR-100 \label{fig:pruning_CIFAR100}]{\includegraphics[width=0.245\linewidth]{figs/pruning_exp/pruning_measure_CIFAR100_resnet50_no_iter.pdf}}
    \subfigure[ImageNet \label{fig:pruning_ImageNet}]{\includegraphics[width=0.245\linewidth]{figs/pruning_exp/pruning_measure_ImageNet_resnet50_no_iter.pdf}}
    \subfigure[Pretrained ViT \label{fig:vit_main}]{\includegraphics[width=0.245\linewidth]{figs/pruning_exp/pruning_measure_CIFAR10_vit_timm_no_iter.pdf}}
    \caption{
    (a, b, c) \textbf{Data pruning experiments.} Test accuracy of the models trained with data subsets of varying ratios in CIFAR-10/100, and ImageNet dataset, selected by different methods. Our method (BWS) outperforms other baselines across a wide range of selection ratios and achieves the accuracy as high as the Oracle window. Full results are reported in Table \ref{tab:CIFAR10_acc}--\ref{tab:ImageNet_acc}. (d) \textbf{Cross-architecture experiments.} Test accuracy of the model fine-tuned with data subsets of varying ratios in the CIFAR-10 dataset, selected by different methods. We utilize the Vision Transformer (ViT) architecture, pretrained on the ImageNet dataset. Our method, BWS, also surpasses other baselines across a wide range of selection ratios. Detailed results are provided in Table \ref{tab:vit_acc}.
    }
    \label{fig:pruning_exp}
\end{figure*}

==> table/ablation/diff_thres.tex <==
\begin{table}
\centering
\caption{Test accuracy of the models trained by window subsets of CIFAR-10 selected by different strategies in choosing the best window subset. Our method consistently achieves the better performance, and the best window subsets selected by ours aligns better with those of oracle windows.
%Test accuracy across various data selection ratios using different window selection strategies. Whereas other methods manifest inconsistent and often poorer outcomes based on the data selection ratio, \ours (kernel ridge regression) consistently shows superior performance across all ratios.
}
\label{tab:diff_thres}
% \vspace{0.2em} 
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|ccccccccc}
\toprule
Selection methods & Selection ratio & 1\% & 5\% & 10\% & 20\% & 30\% & 40\% & 50\% & 75\% & 90\% \\
\midrule
Gradient $\ell_2$-norm & Test accuracy & 54.78 & 81.79 & 87.82 & 90.85 & 91.63 & 92.50 & 93.07 & 94.36 & 94.92 \\
difference    & Window index & 50\% & 45\% & 40\% & 35\% & 30\% & 25\% & 20\% & 10\% & 5\% \\
\midrule
Gradient cosine & Test accuracy & 43.39 & 71.99 & 84.17 & 91.34 & 93.35 & 94.38 & 94.93 & 95.20 & 95.22 \\
  similarity  & Window index & 30\% & 25\% & 20\% & 15\% & 10\% & 5\% & 0\% & 0\% & 0\% \\
\midrule
\multirow{2}{*}{Regression (ours)} & Test accuracy & 63.14 & 81.31 & 88.05 & 91.29 & 93.17 & 94.38 & 94.93 & 95.20 & 95.22 \\
    & Window index & 90\% & 70\% & 35\% & 25\% & 15\% & 5\% & 0\% & 0\% & 0\% \\
\midrule
\multirow{2}{*}{Oracle window} & Test accuracy & 65.73 & 83.03 & 88.05 & 91.69 & 93.35 & 94.38 & 94.93 & 95.20 & 95.22 \\
    & Window index & 80\% & 50\% & 35\% & 20\% & 10\% & 5\% & 0\% & 0\% & 0\% \\
\bottomrule
\end{tabular}}
\end{table}

==> table/ablation/diff_window.tex <==
% 후보군: random, hard-only, easy-only, hard-easy mix, 25~75%, ours, best

\begin{table}
\centering
\caption{Test accuracy of the models trained by different types of window subsets of CIFAR-10.}
\label{tab:diff_window}
\vspace{0.3em} 
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
Selection ratio & Hard-only & Easy-only & Hard-easy & 25-75\% & BWS (ours)  \\
\midrule
10\% & 60.62 & 82.95 & 73.32 & 87.17 & \textbf{88.05}\\
20\% & 81.35 & 85.99 & 81.42 & 89.96 & \textbf{91.29}\\
30\% & 90.84 & 87.51 & 87.44 & 91.11 & \textbf{93.17}\\
40\% & 94.11 & 88.80 & 90.82 & 91.77 & \textbf{94.38}\\
\bottomrule
\end{tabular}}
% \vspace{-0.2em}
\end{table} 


==> table/neural_collapse.tex <==
\begin{table}[ht]
\caption{}
\label{table:neural_collapse}
\vskip 0.15in
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccr}
\toprule
Subset (\%) & 0-20 & 20-40 & 40-60 & 60-80 & 80-100 \\
\midrule
$tr(\Sigma_W\Sigma_B^\dagger)$   & \textbf{0.3892} &  0.1245  &  0.1768 & 0.2425  &  0.3101     \\
\bottomrule
\end{tabular}
}
\end{center}
\vskip -0.1in
\end{table}

==> table/noise_exp.tex <==
\begin{table}
\caption{Test accuracy of the window subset and classification accuracy of solution obtained by solving regression problem with the window subset when data selection ratios are 10\%, 20\%, 30\%, and 40\%.
Index is ranking of the hardest data in the window subset. Value on the top of each row is test accuracy when the window subset is trained, and the value on the middle in each row is regression accuracy derived by the kernel ridge regression problem, and the value on the bottom of each row is noise ratio in the window subset.}
\label{tab:noise_window}
\vspace{0.2em} 
  \centering
  \resizebox{\textwidth}{!}{  
\begin{tabular}{c|cccccccccccc}
\toprule
\multicolumn{1}{c|}{Index} & 0\% & 5\% & 10\% & 15\% & 20\% & 25\% & 30\% & 35\% & 40\% & 50\% & 70\% & 90\% \\
\midrule
        
\multirow{3}{*}{10\%}  & 60.62& 70.52& 76.03& 80.81& 84.17& 85.74& 87.06& \textbf{88.05}& 87.82& 87.28& 84.74& 82.95 \\
              & 56.84 & 61.98 & 64.30 & 65.61 & 66.73 & 67.40 & 67.96 & \textbf{68.38} & 68.35 & 68.07 & 67.70 & 67.40 \\
              & 56.84 & 61.98 & 64.30 & 65.61 & 66.73 & 67.40 & 67.96 & \textbf{68.38} & 68.35 & 68.07 & 67.70 & 67.40 \\
\midrule
            
\multirow{3}{*}{20\%}  & 81.35& 85.84& 89.38& 91.34& \textbf{91.69}& 91.29& 91.15& 90.85& 90.18& 89.30& 86.83& - \\
             & 76.43 & 77.93 & 78.90 & 79.53 & 79.93 & \textbf{79.96} & 79.95 & 79.89 & 79.71 & 79.44 & 78.87 & - \\
              & 76.43 & 77.93 & 78.90 & 79.53 & 79.93 & \textbf{79.96} & 79.95 & 79.89 & 79.71 & 79.44 & 78.87 & - \\
\midrule
            
\multirow{3}{*}{30\%}   & 90.84& 92.82& \textbf{93.35}& 93.17& 92.82& 92.31& 91.63& 91.28& 90.72& 89.66& 87.51& -  \\
             & 83.75 & 84.44 & 84.71 & \textbf{84.74} & 84.70 & 84.58 & 84.48 & 84.33 & 84.18 & 83.97 & 83.64 & -  \\
             & 83.75 & 84.44 & 84.71 & \textbf{84.74} & 84.70 & 84.58 & 84.48 & 84.33 & 84.18 & 83.97 & 83.64 & -  \\
\midrule

\multirow{3}{*}{40\%}    & 94.11& \textbf{94.38}& 93.93& 93.46& 93.03& 92.50& 92.09& 91.38& 90.92& 89.86& -& -  \\
         & 87.91 & \textbf{87.93} & 87.88 & 87.76 & 87.63 & 87.51 & 87.34 & 87.20 & 87.04 & 86.86 & - & - \\
          & 87.91 & \textbf{87.93} & 87.88 & 87.76 & 87.63 & 87.51 & 87.34 & 87.20 & 87.04 & 86.86 & - & - \\
\bottomrule
\end{tabular}}
\end{table} 

